"The struggle is a part of the experience": Engaging Discontents in the Design of Family Meal Technologies

Meals are a central (and messy) part of family life. Previous design framings for mealtime technologies have focused on supporting dietary needs or social and celebratory interactions at the dinner table; however, family meals involve the coordination of many activities and complicated family dynamics. In this paper, we report on findings from interviews and design sessions with 18 families from the Midwestern United States (including both partners/parents and children) to uncover important family differences and tensions that arise around domestic meal experiences. Drawing on feminist theory, we unpack the work of feeding a family as a form of care, drawing attention to the social and emotional complexity of family meals. Critically situating our data within current design narratives, we propose the sensitizing concepts of generative and systemic discontents as a productive way towards troubling the design space of family-food interaction to contend with the struggles that are a part of everyday family meal experiences.

==> 8_YuxingNotes.tex <==
% (Notes for reference) - deleted from background

% - need for holistic studies on family dynamics and family life in domestic HCI, the bigger picture

% - a opportunity to use family conflicts and tensions as lens to probe individual perspectives and otherwise undesirable conversations. Provide valuable insights on how family dynamics are presented in the daily lives of members and what that means for the design of domestic technology.

% - tensions caused by technology use , we proactive take tensions into consideration and probe families to understand how current tensions may influence needs and goals for technological design. And help inform future domestic technology to address such family dynamics.

% [Desjardins2015] - Piratical challenges of situating research within the busy lives of family members, which inspired a diverse set of methodologies as study approaches. Single setting can lead to diverse experiences and expectations for home technology. Called for investigating how individual experiences of the same home can be different and what the differences mean to design for variation under the same theme for home? 

% [Paul and Dourish, back to the shed - contested value of the home]How can we go beyond common assumptions about what the home is in a way that can tell us more about how to design interactive domestic technologies? 

% [Strengers 2019] - smart home research. A growing body of HCI research calls for a shift in focus from the technologies themselves to their situational and social context where their value to “real people” is foregrounded [34, p.3]. 




Deleted notes from findings:
%%First, drawing on our interview study, we situate the complexity of everyday family meal experiences by describing key differences in what each family member--in this paper, namely parents and children-- prioritized and expected in terms of routine meal planning, including deciding nutritional goals, organizing meals, and managing timing challenges. We then detail the disagreements or misalignments around what family meals meant for each person as a social activity and shared ritual of being together. Next, we turn towards describing tensions around the roles and responsibilities associated with the domestic labor of food preparation as experienced by different family members in our study. Finally, highlighting sketches from our co-design sessions, we discuss diverse ways various members of a family envision designing technology as a means of easing these tensions from their point of view.



textbf{Yuxing's design ideas for discussion (@Liz: I'm listing them here as they relate to findings, and will let you pick which one fits better with routine vs. systematic discontents):}

\subsection{Designing for Routine Discontents: Supporting family members to negotiate differences and disagreements}

\textit{[Yuxing--Note: describe your ideas for some design implications for addressing family differences and disagreements in family meal technology connected back to the data in your findings, e.g. how can technology be designed to help mediate tensions/discontents? Does this involve seeing tensions as a everyday part of life, or even generatively as the way children naturally learn to define their roles in family and have power] }



[Design idea 1:Systems can approach potential tensions, conflicts, and bias by facilitating and scaffolding the process of sharing, communicating and mediating these discontents through co-creation of goals and expectations for the experience. ]

Our finding shows that routine discontent can happen in various parts of the family meal process, from the importance of healthy eating, deciding when to serve a meal, to what is valued in an enjoyable and meaningful family meal (as described in 4.1). As we saw from the Spencer family and the Green family, many factors can impact how everyday tensions around meal planning and preparation arise and cause stress and frustration within the family. As parents in the family (e.g., Jane and Dave from the Spencer Family) discussed their individual views on healthy eating, the distinct opinions new to the parents themselves--for many families, they reported how they find other family members' answers were unexpected and they "learned something new about each other." This suggested one way for mediating these routine discontents through forming common knowledge that the entire family agrees on.

One way to help with mediating tensions is by scaffolding the process of sharing and communicating needs, goals and expectations of what families each look for and setting up guides and rules to follow that are unique for their family to create an enjoyable and meaningful family meal experience. By encouraging family members to share their goals and expectations explicitly, members are prompted to clarify and discuss needs and perspectives that might otherwise have been overlooked in their busy everyday lives. For example, designers could provide instruments to facilitate shared conversations, allowing families to discuss what individual members want and look forward to in a family meal to form mutual understanding. These discussions could feel awkward or unnatural in, say, a pamphlet form, but interactive HCI and CSCW technologies hold the potential to mediate family expectation-setting and role-distribution activities in fun and engaging ways. For example, interactive technology can be designed to link with individual schedules and suggest weekly collaborative family meal activity--where each family member is asked to work to co-create rules and expectations for the experience in a gaming format (e.g., what to eat, when the family meal tasks place and for how long). To help with decisions and coming to an agreement as a family, for each activity, one family member is selected as the "family meal lead" who gets to make the "ultimate decision" when balancing differing goals and needs within the family. This role can be rotated to ensure everyone gets a chance to be the lead. In scaffolding the process of co-creation of family meal as a team, we see design opportunities for seeing tensions as part of everyday life of families that can be mediated through intentional collaborative family activities and conversations. 

[Not sure where to put this, but feels important to acknowledge] Meanwhile, we acknowledge that tensions, especially routine discontents are common in everyday practices and is part of what it means to navigate the domestic life. The goal of technology should not be to "eliminate" tensions, rather, providing families the medium to feel comfortable to share their unique views and talk about how their opinions on certain topics are different from each other, and that's okay.

[Design idea 2: Support father and children/siblings co-learning to cook ]

There is also an opportunity for design to encourage family members’ (especially children’s) participation from a learning perspective. HCI and CSCW communities have looked at parents’ roles in family interactions, but mostly in learning and education [8,24,102]. Prior work showed that understanding and considering parents’ roles will support learning, such as coding and AI literacy, for not only the kids but the entire families as well [24,102]. In our study, we answered Barron’s call for examining parents’ roles in other environments. We demonstrated how understanding roles and their corresponding values for all family members is crucial for designing collaborative family meal experiences. Unlike content knowledge learning at school or self-directed learning at home, meal preparation (cooking) may not be a typical skill that parents or kids explicitly learn (e.g., as opposed to learning math), but it is still a well-recognized, important life skill. Teaching and learning to cook are often embedded in the natural day-to-day family meal practices, which are often overlooked due to busy schedules or lack of interest from children. Many parents intend to prepare their kids to be able to cook, but are either too busy to do it or may not be confident in guiding kids in cooking (especially parents who are not the main meal preparer, as described in 4.2). 

\textit{Support role flexibility through co-learning for parents and children}
In most families, the mother took up the role of meal preparer. Many parents, especially the father, have very limited time for participating in meal preparation (as described in 4.2). As a result, they may be unfamiliar with cooking for the family and even miss the family meals as an opportunity to connect with the child(ren) (e.g., cite family). Technology should consider supporting the co-learning experience for parents and children where they can cook together. For example, an interactive system can provide families with a step-by-step video tutorial of how parents and children may collaborate together on a dish (e.g., the kid washes the tomatoes and the parent cut them into thin slices). Different than a traditional cooking tutorial, the system can add prompts and discussion points throughout the activity as fun facts on an ingredient, and open up conversations between parents and children (e.g., Tomatoes were originally considered poisonous by all but a few Americans until the mid-1800s[107]. What was a time when you tried/did something that most people would not do? What was that like and how did you feel about it?). Such features will not only meet parents’ (especially the ones who seldom cook) desire to have more time to connect with kids (e.g., Dad from F2), but can also engage children in interesting activities through family co-learning to help spark interest. By scaffolding the social interactions during the process of cooking together, the system can also support family communication and bonding. However, such scaffolding features should balance children’s needs/willingness for parents’ support with cooking and parents’ desire for children’s ability to cook independently. How the features can adapt with child development over time or how it should negotiate the balance between scaffolding and independence require more exploration in future research [102].

\textit{Designing for sibling interactions}
14 out of 18 families reported having more than one child and seeing different interests in meal prep between siblings. For example, (F5 kid?) who was older had a passion for cooking and wanted more opportunities to engage in meal prep (as described in 4.2.2). However, her younger brother did not share the same interest and had not thought much about cooking. There is an opportunity for technology to support collaborative cooking interactions. Following Go et al. and Yu et al.’s design suggestions for sibling play [38,102], we recommend that: (1) given the ability and interest differences between siblings, technology should consider the different levels of difficulty and assign different tasks based on the age and capabilities among the siblings; (2) since sibling often acts as scaffolders for each other [38], design can include play mechanisms that support the older sibling acting as a scaffolder to the younger one(s), such as showing how to make a sandwich and inspiring each other how to change the fillings to create different flavors in a shared cooking experience. From a learning perspective, such shared engagement features can also help siblings to inspire cooking interests in each other and support parents’ desires in the children to learn an important life skill.

There are also opportunities for family members (especially siblings) to learn how to deal with differences and minor tensions during such co-learning of cooking...how to negotiate with each other and form a mutual understanding and agreement on things. 


[Design idea 3: Supporting emerging technology to adapt to different roles given the different process, context and family members involved during meal experience]

As described in 4.3, mothers, fathers and children tend to expect technology to support different parts of the family meal process--the functional vs. social vs. playful aspect (cite). They also described different levels of comfort of how they see technology in existing meal practices and how they perceive technology to play what role: 

- Assistance/helper for moms
- mediator/facilitator for dads
- playmate/ instructor/companion for kids

Design recommendation: Attending to the different comfort levels of how each family member want tech to be involved. Support changing roles (flexibility in roles) in tech. [cite robot paper] - Challenges of existing meal technologies on acceptance and long-term engagement
One way of supporting different levels of control and automation with smart home technology is through changing the role of technology as it situates in different context 
e.g., (examples in family envions different role technology plays in meal process) - design systems that can adapt and change its "role" by changing settings: Imagine a kitchen robot--Prorities is based on the main preparer as the default setting, but with customizable options for equitable access and control in the family. [cite Bengisu - robot in the home].



-------------ignore notes below--------------

e.g. Rotating a "meal lead" in the family to decide and help plan the menu

There is also an opportunity for design to encourage family members’ (especially children’s) participation from a learning perspective. 

1. Support changing roles/flexibility of roles in technology 

- provides a set of adaptive roles for tech to reflect family members' preferences in different meal processes, as well as different users for the activity.



e.g., (examples in family envions different role technology plays in meal process) - design systems that can adpat and change its "role" by changing settings: Imagine a kitchen robot--Prorities is based on the main preparer as default setting, but with customizable options for equitable access and control in the family. [cite Bengisu - robot in the home]

2. Support co-learning/co-expereince to share and collaborate on meal processes
- leveraging difference to promote sibling interaction (cite example in data: One child is interested to cooking while the other is not)


[Design implication for attending to the family dynamics and tensions around diverse needs, values and roles]
- address family dynamics and tensions more proactively

- Meal prep as a gendered role
- Encourage and prompt families to come up with goals and shared roles as a group
- system with default priorities (e.g. healthy eating, timeliness, meal conversation)

These differences are surprising for families themselves 

one way is to design around the roles that each family member plays in the experience. 

"co-experience" of family members

HCI research tends to focus on 

- factors/sources of disagreement and conflict [build on Detrix - family tech use as sources of conflict for parents]

https://dl.acm.org/doi/10.1145/2470654.2481365

- Reflect on meal technology - failed support long-term engagement and acceptance

- Collaborate and in control of technology use 






% Please insert any discussion ideas that you may have!

% From Yuxing's previous discussion note:

% While meals are a time to gather together, differences, disagreements, and conflicts (however small) are still common and must be considered in the design of family meal technologies. Our findings showed that within a family, members may hold different and even conflicting on various aspects of family meals, including what they prioritize and value for a family meal, what roles they take on and expect from each other, and how they perceive technology to support our future meal experiences. These differences and conflicts not only can create tensions between family members, but more importantly, can challenge and impact how well technology can be accepted and integrated into the domestic lives of the family in a meal setting. Design of family meal technology that ignores these tensions and differences may be at their peril. 

% In this section, we discuss design recommendations for future meal technologies based on the findings. 

% % In this section, we reflect on the use of family differences and disagreements for understanding family dynamics (benefits and potential drawback+cautions) and design recommendations for domestic technology in meal context (existing meal tech failed to support or why families abandoned them) (and beyond?), and discuss challenges faced in understanding family as a whole and potential tactics for exploring family members' differing perspective. (research tactics in terms of methods to engage with families as a group, use of remote method, group activities and probing design activity in co-design session with family)

% \subsection{Supporting family members to share, communicate, and negotiate differences and disagreements}

% [Design implications for addressing family differences and disagreements in family meal technology]

% - provides a set of adaptive roles for tech to reflect family members' preferences in different meal processes, as well as different users for the activity.

% - Assistance/helper for moms
% - mediator/facilitator for dads
% - playmate/ instructor/companion for kids

% [Design implication for attending to the family dynamics and tensions around diverse needs, values and roles]
% - address family dynamics and tensions more proactively

% - Meal prep as a gendered role
% - Encourage and prompt families to come up with goals and shared roles as a group
% - system with default priorities (e.g. healthy eating, timeliness, meal conversation)



% These differences are surprising for families themselves 

% one way is to design around the roles that each family member plays in the experience. 

% "co-experience" of family members

% HCI research tends to focus on 

% - factors/sources of disagreement and conflict [build on Detrix - family tech use as sources of conflict for parents]

% https://dl.acm.org/doi/10.1145/2470654.2481365

% - Reflect on meal technology - failed support long-term engagement and acceptance

% - Collaborate and in control of technology use 

% \subsection{Using family disagreements and conflicts to inform how meal technology might be integrated in domestic environments to support shared family activities}

% 1. Importance and benefits of understanding family disagreements - explores the dynamics of needs and expectations for individual family members. This is helpful not only for meal technology but for understanding and designing domestic technology that sits in the home (e.g., smart-home technology and in-home robots) 

% 2. However, HCI community has focused on individual members rather than family as a whole. How researchers may dive into the entangled needs and values of family members and come up with design suggestions that attend to the diverse individual expectations, attitudes and roles is unclear. Efforts 

% complex experience of family technology use 

% - tactics
% - Methods and challenges


% HCI research involving families has primarily focused on individual family members, rather than family as a whole. 

% - design implication and recommendation for meal technology
% - benefits 

% Holistic, nuanced experience of family experiences with technology 

% Our paper presented a case of how family difference and conflicts can be surfaced in the case of shared family meals. 
 
% explore family experience 

% Benefits of investigating families as a whole: 1. helps with surfacing family dynamics that impact technology acceptance and 
% 2. created opportunities for conversation between members and to shift their individual perspectives 3. enable reflection of socially undesirable, uncomfortable situations and scaffold discussion of social and gendered dynamics of roles

% These differences and conflicts can create tensions between family members and challenge family coordination and collaboration methods, and even parenting philosophy. Design of family meal technologies that ignores these tensions and differences may be at their peril.

% When designing for family as a group, it is imperative to consider individual goals and priorities. Researchers have emphasized the need to understand individual goals and experiences during collaborative interactions [18,77,81]. Of particular note are Panicker and colleagues’ calls to incorporate individual and family goals when designing for family informatics systems [77].
% Our findings reinforce the importance of unpacking the “family space” and confirm the value of investigating how and why family members develop and change their goals and expectations. Many tensions we saw in the study centered on the roles around meal preparations: (1) The main meal preparer experienced role strains and wanted to reduce the stress (as described in 4.3.1), yet busy family routines and institutional norms may limit families’ ability to delegate the role (as shown in 4.2.1); (2) The degree to which kids should be involved in meal prep and become competent in the preparer role. For example, parents and kids had different motivations and thoughts on using meal preparation as an opportunity

% 1. Talk about design implications for domestic technology in family meal context as a common shared family activity - support collaboration beyond data access and sharing, tracking. Dive into the needs and values and the dynamics that impact the usage and different interactions that different families will have with the technology. 
% This is particularly important for designing for family as a whole and help us understand and support acceptance and long-term engagement.

% - demand for meal technology beyond use or non-use

% Based on our findings, what are some main design considerations - factors and sources for disagreement.

% Given the specific design space and context, it's up to the designers and researchers to decide which needs or values 

% Expanding the definition of family meal allowed family members to elaborate on their needs beyond the act of having meal itself and presented design opportunities 

% We call for future family meal technology to embrace

% Reconsider technology we introduce in family meal experiences. Understanding 

% Supporting dynamics and expectations around roles and role transitions: Based on the differences in desired roles of the family meal technology, we suggest designers incorporate an adaptive set of roles for the robot reflecting family members’preferences.

% - the smartness of technology
% Many of the families imagined smart kitchen or AI-powered technology to help with different aspects of their meal process. 
% - family dynamics such as social and gender dynamics around values and roles 

% - Designers should acknowledge and consider such dynamics and differences in creating domestic technology when identifying commonalities in design.

% design recommendations:


% [Cagiltay1, in-home robot, full paper]"Design Recommendations. While not two families completely agreed on one set of priorities, the unique dynamics of each family revealed the need for family-controlled settings. Through carefully curated user profiles, parents and children would benefit from having the option to set boundaries, limitations, house rules, and family hierarchy preferences. For maintaining authority, as families (F1, F3, F5, and F7) suggested, we recommend designers to provide default parent privileges for interactions, which parents can access and adjust through user profiles and authentication methods, such as face recognition. However, it is also crucial for designers to seek equitable ways to provide authority settings while maintaining the trust and bond between the child and the robot. For example, the robot should not impose family rules on the child but take a peer-like approach by suggesting and reminding pre-set house rules and authority settings. To resolve priority conflicts in group interactions, we suggest designers to provide default settings for the robot to manage the priorities of group members, along with options for users to personalize these priorities. These settings can include scheduling options such as first-come-first-served or priority queues based on the activity type and time spent on each interaction per family member. Additionally, adaptive feedback mechanisms to improve family-specific priority management over time can be beneficial for the acceptance of the robot in long-term interactions."

% More comprehensive understanding of the individual and joint needs of parents and children in smart home 

% AI and smart home - algorithm design. Family-centric 

% Reflect on previous meal technology 
% - [Ferdous, celebratory technology] how these technologies can be meaningfully integrated into family practices

% privacy and safety concerns for home robots and AI tech - from the quote "it's creepy"

% position statement: we focused on family meal in our study. Although there are different needs and impact factors in other shared family contexts, we think takeaways and insights is transferable in 

% (tech lead in the family)

% 2. Talk about ways to capture, surface and actively probe for differences 
% [show must go on]


% ----------


% \subsection{Strategies to probe for diverse goals and expectations and design for the family as a whole}

% - power dynamics
% - from child-centered to family-centered 


% 1. Importance of considering disagreements and differences when designing for shared family experiences
% - Family systems have been adopted and abandoned. Why is that? 

% - What does it mean to design domestic technology?

%  - We should consider the potential differences and disagreements that can lead to no matter how nuanced they are.

%  - understanding and addressing the gender and social dynamics in 

% 2. Ways of designing for surfacing, communicating, and resolving family disagreements 
 
%  - designing technology that supports the \textit{process} of sharing and communicating individual views, goals, and values. Help families to create norms and values that everyone contributes, agrees, and adheres to. 

 
% - tactics for probing differences and disagreements among families
%  - group activity and discussions as a way to address power dynamics

% - There are few Negotiation and attempts to resolve disagreements (F1, F2)
%  - Not all disagreements are bad


% \subsection{Conducting synchronous participatory design with families online}

% - reflecting on how to work with family as a group

% cite Yip's the show must go on
% challenges on working with both parents and children at the same time




% ------
% family perception and needs for technology are influenced and entangled with their roles and dynamics in the family. Our paper presents the complexity of addressing different and sometimes conflicting goals and values in the case of family meal technologies. We also reflect on the factors that impact 

% What is our RQs? (intro)


% What is our motivation for studying family differences, disagreements, and tension?

% Why should the HCI community care about this?

% How might HCI researchers and designers consider and incorporate differences and disagreements when working and designing technology for families?

% - How has previous work address differences and disagreements for family technology

% -----
% From a family wellness standpoint, there is a design opportunity to support the surfacing and communication of differences and disagreements. 
% - how technology can be used to encourage and bring more family conversations to share and learn about each others' 
% - Provide a safe space 

% ----
% From a design/system perspective, whose desires, goals and values are/should we prioritize?

% differences in intended usage

% We said that we need to include children (grandparents, extended family members etc.) in designing for the family, but what does that mean when each stakeholder want different things? How to align the differences?

==> Accessbility.tex <==
Figure 1a:  "This is a picture of the design sketch from Jen (mother from the Chen Family). The sketch shows an envisioned smart kitchen where she can complete the steps of planning, shopping and cooking a meal through the help of the system"
Figure 1b: "This is a picture of the design sketch from Dave (father from the Spencer Family). In the sketch, Dave is wearing a VR headset that allows him to connect with his extended family members while eating pills as his dinner."
Figure 1c: "This is a picture of the design sketch from Hannah (daughter from the White Family). She imagined a game called 'Dinner Quest' that allows her and her family to compete against each other to win points during a family dinner."
Figure 2a: "This is a picture of the design sketch from Emma (mother from the Jean Family). She drew out a fully automated smart kitchen that handles everything for making a meal, from ordering groceries, cooking, serving the dishes to the table, and cleaning up."
Figure 2b: "This is a picture of Claude’s design sketch. He drew out a scenario where everyone in his family is having an engaging conversation over food. He noted on the sketch that his ideal family dinner would be limited use of technology with 'No TV' and 'No Phones', and everyone help with cleaning up."
Figure 2c: "This is a picture of the design sketch from Jess (child from the Jean Family). He drew a humanoid home robot that can help with all kinds of tasks and is designed for assistance and companionship in the home. The robot has a head, two arms and hands, and wheels as its leg for moving around the house."

Table 1: "This is a participant table detailing family demographics. It lists 18 families with children as our study participants. All participants are anonymized with IDs and pseudonyms. There are 18 rows and 5 columns. The column headers from left to right are: Family, Race/Ethnicity, Parent(Gender, Age), Children (Gender, Age), and Household Income."
